Future prospects for exploring present day anomalies in flavour physics measurements with Belle II and LHCb

A range of flavour physics observables show tensions with their corresponding Standard Model expectations: measurements of leptonic flavour-changing neutral current processes and ratios of semi-leptonic branching fractions involving different generations of leptons show deviations of the order of four standard deviations. If confirmed, either would be an intriguing sign of new physics. In this manuscript, we analyse the current experimental situation of such processes and for the first time estimate the combined impact of the future datasets of the Belle II and LHCb experiments on the present tensions with the Standard Model expectations by performing scans of the new physics contribution to the Wilson coefficients. In addition, the present day and future sensitivity of tree-level CKM parameters, which offer orthogonal tests of the Standard Model, are explored. Three benchmark points in time are chosen for a direct comparison of the estimated sensitivity between the experiments. A high complementarity between the future sensitivity achieved by the Belle II and LHCb experiments is observed due to their relative strengths and weaknesses. We estimate that all of the anomalies considered here will be either confirmed or ruled out by both experiments independently with very high significance by the end of data-taking at Belle II and the LHCb upgrade.

==> gamma.tex <==
\section{CKM angle $\gamma$}
\label{sec:gamma}

\textcolor{red}{\textit{Matt}}

